TransText: Alpha-as-RGB Representation for Transparent Text Animation

We introduce the first method, to the best of our knowledge, for adapting image-to-video models to layer-aware text (glyph) animation, a capability critical for practical dynamic visual design. Existing approaches predominantly handle the transparency-encoding (alpha channel) as an extra latent dimension appended to the RGB space, necessitating the reconstruction of the underlying RGB-centric variational autoencoder (VAE). However, given the scarcity of high-quality transparent glyph data, retraining the VAE is computationally expensive and may erode the robust semantic priors learned from massive RGB corpora, potentially leading to latent pattern mixing. To mitigate these limitations, we propose TransText, a framework based on a novel Alpha-as-RGB paradigm to jointly model appearance and transparency without modifying the pre-trained generative manifold. TransText embeds the alpha channel as an RGB-compatible visual signal through latent spatial concatenation, explicitly ensuring strict cross-modal (RGB-and-Alpha) consistency while preventing feature entanglement. Our experiments demonstrate that TransText significantly outperforms baselines, generating coherent, high-fidelity transparent animations with diverse, fine-grained effects.

==> sections/abs.tex <==
\begin{abstract}

We introduce the first method, to the best of our knowledge, for adapting \emph{image-to-video} models to layer-aware text (glyph) animation, a capability critical for practical dynamic visual design.
Existing approaches predominantly handle the transparency-encoding ($\alpha$ channel) as an extra latent dimension appended to the RGB space, necessitating the reconstruction of the underlying RGB-centric \emph{variational autoencoder} (VAE).
However, given the scarcity of high-quality transparent glyph data, retraining the VAE is computationally expensive and may erode the robust semantic priors learned from massive RGB corpora, potentially leading to latent pattern mixing.
To mitigate these limitations, we propose \textbf{TransText}, a framework based on a novel \emph{Alpha-as-RGB} paradigm to jointly model appearance and transparency without modifying the pre-trained generative manifold. 
\textbf{TransText} embeds the $\alpha$ channel as an RGB-compatible visual signal through latent spatial concatenation,  
explicitly ensuring strict cross-modal (RGB-and-Alpha) consistency while preventing feature entanglement. Our experiments demonstrate that \textbf{TransText} significantly outperforms baselines, generating coherent, high-fidelity transparent animations with diverse, fine-grained effects.

\end{abstract}

% , yielding temporally coherent and high-fidelity transparent animations characterized by diverse, fine-grained visual effects.

% This paper presents the first study dedicated to adapting \emph{image-to-video} (I2V) frameworks for high-fidelity layer-aware text (glyph) animation, a critical capability for practical dynamic visual design. 
% Existing approaches predominantly handle the transparency-encoding ($\alpha$ channel) as an extra latent dimension appended to the RGB space, necessitating the reconstruction of the underlying RGB-centric \emph{variational autoencoder} (VAE).
% However, given the scarcity of high-quality transparent glyph data, such retraining not only incurs substantial computational overhead but also degrades the robust semantic priors established on billion-scale RGB corpora, risking latent pattern mixing.
% To tackle these limitations, we propose \textbf{TransText}, a framework that introduces a novel \emph{Alpha-as-RGB} paradigm to unify appearance and transparency without altering the pre-trained generative manifold. 
% Specifically, \textbf{TransText} embeds the $\alpha$ channel as an RGB-like intrinsic visual signal via latent spatial concatenation, explicitly ensuring strict cross-modal (RGB-and-Alpha) consistency while preventing feature entanglement.
% Extensive experiments demonstrate that \textbf{TransText} significantly outperforms existing baselines, generating temporally coherent, high-fidelity transparent animations featuring diverse and fine-grained visual effects.


% This paper presents the first study of adapting \emph{image-to-video} (I2V) framework dedicated to high-fidelity glyph animation with transparency (Alpha-layered). Existing RGB-centric approaches addressing Alpha typically graft transparency onto RGB diffusion generalists by reconstructing the latent space, necessitating computationally expensive \emph{variational auto-encoder} (VAE) retraining. 
% However, given the scarcity of high-quality RGBA glyph data, this retraining process inevitably degrades the robust semantic priors of billion-scale foundation models, leading to diminished fidelity and temporal inconsistency. 
% In this case, we propose \textbf{TransText}turn to a novel \emph{Alpha-as-RGB} paradigm that unifies appearance and transparency into a single representation without altering the generative manifold. 
% Specifically, \textbf{TransText} embeds the alpha channel directly within the RGB space via \emph{Latent Spatial Alignment}, treating transparency as an intrinsic visual signal. 
% By spatially concatenating RGB and alpha latents, our framework explicitly enforces strict cross-modal alignment throughout the diffusion process while preventing feature entanglement. Additionally, 
% this design is further fortified by a fine-grained regularization term to ensure precise structural boundary definition. 
% Extensive experiments demonstrate that our framework generates temporally coherent, high-fidelity RGBA text animations with precise opacity control and no color leakage.
% It also significantly outperforms existing baselines in both generation quality and structural accuracy.





% Generating transparent (alpha-layered) videos for \textname~animation is a crucial capability for digital typography, AR/VR interfaces, and motion graphic design. 
% % However, existing \emph{image-to-video} (I2V) diffusion models struggle with this task: they either neglect transparency entirely or rely on VAE-based frameworks that decouple RGB and alpha channels, resulting in motion misalignment and severe RGB-alpha mixing artifacts. 
% However, existing \emph{image-to-video} (I2V) diffusion models either neglect transparency entirely or rely on VAE-based frameworks that decouple RGB and alpha channels.
% This decoupling results in motion misalignment and severe RGB-alpha mixing artifacts. 
% To address this limitation, we present \textbf{TransText}, the first I2V framework that unifies appearance and transparency into a single representation. 
% % Unlike prior approaches that require separate latent encoders, we propose an \emph{Alpha-as-RGB} strategy that treats the alpha channel as an intrinsic visual signal embedded directly within the RGB space. 
% \textbf{TransText} embeds the alpha channel directly within the RGB space as an intrinsic visual signal. 
% % Our method employs spatial concatenation to explicitly align RGB and alpha learning throughout the diffusion process, further enhanced by alpha-aware attention mechanisms and a dedicated regularization term. 
% This direct embedding is achieved by a spatial concatenation in the latent space, which explicitly aligns RGB and alpha learning throughout the diffusion process. 
% The alignment is further enhanced by alpha-aware attention mechanisms and a dedicated regularization term. 
% Extensive experiments demonstrate that our framework generates temporally coherent, high-fidelity RGBA text animations with precise opacity control and no color leakage.
% It also significantly outperforms existing baselines in both generation quality and structural accuracy.

